Self-Activating Neural Ensembles for Continual Reinforcement Learning

The ability for an agent to continuously learn new skills without catastrophically forgetting existing knowledge is of critical importance for the development of generally intelligent agents. Most methods devised to address this problem depend heavily on well-defined task boundaries, and thus depend on human supervision. Our task-agnostic method, Self-Activating Neural Ensembles (SANE), uses a modular architecture designed to avoid catastrophic forgetting without making any such assumptions. At the beginning of each trajectory, a module in the SANE ensemble is activated to determine the agent's next policy. During training, new modules are created as needed and only activated modules are updated to ensure that unused modules remain unchanged. This system enables our method to retain and leverage old skills, while growing and learning new ones. We demonstrate our approach on visually rich procedurally generated environments.

==> dump.tex <==


\subsection{Future Extensions}

We kept the design of SANE as straightforward as possible in this paper, but there are a couple of natural extensions we believe make the method even more general and robust that will be investigated in future work.

\noindent {\bf More frequent activation:} Instead of collecting a batch of trajectories, in principle a new node could be selected every timestep, using the latest observation instead of the first observation of the episode. This more frequent update would allow each module to represent a finer-grained behavior, which would likely be more re-usable and enable more forward transfer.

However in practice we found this to be infeasibly slow. As compute improves, or as we move into environments where data collection is the bottleneck (such as real-world robotics tasks), we believe this assumption may be relaxed.

\noindent {\bf Hierarchical representations:} There are a few downsides to a single-layer ensemble. Most notably, while on one hand you might want a very large ensemble to capture many different behaviors, this increases the number of critics that need to be kept accurate to activate their modules appropriately. Additionally, this increases the number of critics that must be evaluated each time you wish to activate a node. These can be addressed by making a hierarchy of modular critics, where instead of a single activation, a path of critics through the tree is activated, each building upon the representation of the node above it.




\subsection{Activation Metric}
\label{section:activation}
By design our concept of an activation metric is quite general. Any network designed for any task that may experience drift can benefit from the modularization our self-activating modules provide. The one assumption necessary is that there must be some form of feedback as to whether the network is performing well or not, in other words some success metric. As an example, a world model might used a metric based on predictive accuracy: an outcome of some action is predicted, and the success metric is how accurate that prediction was. A voice recognition network, designed to perform some set of actions when instructed to verbally, might use a success metric based on repetition: how many times in a short span the person repeats themselves. For RL, the metric may simply be the total reward received from the environment during an episode.

Given such a success metric, we can modularize the network by creating an ensemble of networks that solve the task, each augmented with another network that estimates the success metric expected if that module is activated. We term the estimate of this success metric our \emph{activation metric}. In the case of reinforcement learning, the activation metric already has a name: a critic, as in the actor-critics described above, which we will use going forward to reflect our primary focus in this paper on the CRL setting. Note that we adjust the standard critic slightly to encourage exploration, discussed further in Section \ref{section:primitive}.

The one requirement for SANE to work well is that this critic be as accurate as possible. This is important for four key reasons. First, when an agent starts learning a new task, a module tailored to an old task will activate. The critic of this module must make predictions accurate to the new setting before the policy learns a new behavior, so a new module is created before the old behavior is overwritten. Second, the critic should not overfit to a particular task such that it always predicts a high value regardless of what task it is being used on. This is particularly important given the continual evaluation protocol described in Section \ref{section:crl_setting}, where we do not update the ensemble during evaluation, which prevents the critic from adapting to any unexpectedly low rewards. Third, a noisy critic will lead to slower learning: if a particular task might activate one of several different modules, learning is slowed as each module learns the same information separately. Fourth, an inaccurate critic will detect drift incorrectly, resulting in the creation of new modules unnecessarily.

One additional key aspect is that the computation of a module's activation metric should be untouched while training other modules; every node in our ensemble is completely isolated from all others to minimize catastrophic forgetting, and this should extend to the activation metric as well. 

\sam{Somewhere discuss tradeoff between more nodes/smaller buffer vs fewer/larger buffer}
